SALSA-CLRS: A Sparse and Scalable Benchmark for Algorithmic Reasoning

We introduce an extension to the CLRS algorithmic learning benchmark, prioritizing scalability and the utilization of sparse representations. Many algorithms in CLRS require global memory or information exchange, mirrored in its execution model, which constructs fully connected (not sparse) graphs based on the underlying problem. Despite CLRS's aim of assessing how effectively learned algorithms can generalize to larger instances, the existing execution model becomes a significant constraint due to its demanding memory requirements and runtime (hard to scale). However, many important algorithms do not demand a fully connected graph; these algorithms, primarily distributed in nature, align closely with the message-passing paradigm employed by Graph Neural Networks. Hence, we propose SALSA-CLRS, an extension of the current CLRS benchmark specifically with scalability and sparseness in mind. Our approach includes adapted algorithms from the original CLRS benchmark and introduces new problems from distributed and randomized algorithms. Moreover, we perform a thorough empirical evaluation of our benchmark. Code is publicly available at https://github.com/jkminder/SALSA-CLRS.

==> results/algorithmwise/bfs_node_f1.tex <==
\begin{tabular}{llrrrrrr}
\toprule
\bottomrule
\end{tabular}


==> results/algorithmwise/dfs_node_f1.tex <==
\begin{tabular}{llrrrrrr}
\toprule
\bottomrule
\end{tabular}


==> results/algorithmwise/dijkstra_node_f1.tex <==
\begin{tabular}{llrrrrrr}
\toprule
\bottomrule
\end{tabular}


==> results/algorithmwise/mst_prim_node_f1.tex <==
\begin{tabular}{llrrrrrr}
\toprule
\bottomrule
\end{tabular}


==> results/graph_accuracy_old.tex <==
\resizebox{.9\textwidth}{!}{
\begin{tabular}{l@{\hspace{1em}}l@{\hspace{1em}}S[table-format=3.1]@{\hspace{2.5em}}S[table-format=3.1]@{\hspace{2.5em}}S[table-format=3.1]@{\hspace{2.5em}}S[table-format=3.1]@{\hspace{2.5em}}S[table-format=3.1]@{\hspace{4em}}S[table-format=3.1]@{\hspace{2.5em}}S[table-format=3.1]@{\hspace{2.5em}}S[table-format=3.1]@{\hspace{2.5em}}S[table-format=3.1]@{\hspace{2.5em}}S[table-format=3.1]@{\hspace{4em}}S[table-format=3.1]@{\hspace{2.5em}}S[table-format=3.1]@{\hspace{2.5em}}S[table-format=3.1]@{\hspace{2.5em}}S[table-format=3.1]@{\hspace{2.5em}}S[table-format=3.1]@{\hspace{2.5em}}}
\toprule
    &        & \multicolumn{5}{l}{ER} & \multicolumn{5}{l}{WS} & \multicolumn{5}{l}{Delaunay} \\
    &        &   \multicolumn{1}{l}{16}   &  \multicolumn{1}{l}{80}   &  \multicolumn{1}{l}{160}  &  \multicolumn{1}{l}{800}  &  \multicolumn{1}{l}{1600}  &   \multicolumn{1}{l}{16}   &  \multicolumn{1}{l}{80}   &  \multicolumn{1}{l}{160}  &  \multicolumn{1}{l}{800}  &  \multicolumn{1}{l}{1600} &     \multicolumn{1}{l}{16}   &  \multicolumn{1}{l}{80}   &  \multicolumn{1}{l}{160}  &  \multicolumn{1}{l}{800}  &  \multicolumn{1}{l}{1600} \\
\midrule
bfs & GIN(E) &  100.0 \text{\tiny $\pm$ 0.0} &   91.0 \text{\tiny $\pm$ 7.5} &  64.1 \text{\tiny $\pm$ 18.8} &    3.6 \text{\tiny $\pm$ 6.5} &    0.3 \text{\tiny $\pm$ 0.5} &  100.0 \text{\tiny $\pm$ 0.0} &  11.7 \text{\tiny $\pm$ 14.5} &    0.3 \text{\tiny $\pm$ 0.6} &   0.0 \text{\tiny $\pm$ 0.0} &   0.0 \text{\tiny $\pm$ 0.0} &  100.0 \text{\tiny $\pm$ 0.0} &  57.2 \text{\tiny $\pm$ 19.3} &    4.8 \text{\tiny $\pm$ 5.6} &  0.0 \text{\tiny $\pm$ 0.0} &  0.0 \text{\tiny $\pm$ 0.0} \\
        & RecGNN &   99.9 \text{\tiny $\pm$ 0.1} &   92.7 \text{\tiny $\pm$ 3.1} &  64.0 \text{\tiny $\pm$ 12.6} &    2.2 \text{\tiny $\pm$ 2.6} &    0.1 \text{\tiny $\pm$ 0.2} &  100.0 \text{\tiny $\pm$ 0.0} &  22.1 \text{\tiny $\pm$ 15.3} &    1.0 \text{\tiny $\pm$ 1.2} &   0.0 \text{\tiny $\pm$ 0.0} &   0.0 \text{\tiny $\pm$ 0.0} &  100.0 \text{\tiny $\pm$ 0.0} &  46.5 \text{\tiny $\pm$ 26.5} &  10.4 \text{\tiny $\pm$ 15.2} &  0.0 \text{\tiny $\pm$ 0.0} &  0.0 \text{\tiny $\pm$ 0.0} \\
bfs (H) & GIN(E) &  90.4 \text{\tiny $\pm$ 18.7} &  58.5 \text{\tiny $\pm$ 36.2} &  33.1 \text{\tiny $\pm$ 24.7} &    0.8 \text{\tiny $\pm$ 0.9} &    0.0 \text{\tiny $\pm$ 0.1} &  90.1 \text{\tiny $\pm$ 18.3} &    2.1 \text{\tiny $\pm$ 2.2} &    0.0 \text{\tiny $\pm$ 0.0} &   0.0 \text{\tiny $\pm$ 0.0} &   0.0 \text{\tiny $\pm$ 0.0} &  82.7 \text{\tiny $\pm$ 35.3} &    1.3 \text{\tiny $\pm$ 1.1} &    0.0 \text{\tiny $\pm$ 0.0} &  0.0 \text{\tiny $\pm$ 0.0} &  0.0 \text{\tiny $\pm$ 0.0} \\
        & RecGNN &   99.5 \text{\tiny $\pm$ 0.4} &  62.0 \text{\tiny $\pm$ 17.1} &  22.9 \text{\tiny $\pm$ 14.1} &    0.0 \text{\tiny $\pm$ 0.1} &    0.0 \text{\tiny $\pm$ 0.0} &   99.0 \text{\tiny $\pm$ 1.9} &    2.1 \text{\tiny $\pm$ 2.1} &    0.0 \text{\tiny $\pm$ 0.1} &   0.0 \text{\tiny $\pm$ 0.0} &   0.0 \text{\tiny $\pm$ 0.0} &   99.0 \text{\tiny $\pm$ 1.3} &    0.1 \text{\tiny $\pm$ 0.1} &    0.0 \text{\tiny $\pm$ 0.0} &  0.0 \text{\tiny $\pm$ 0.0} &  0.0 \text{\tiny $\pm$ 0.0} \\
\midrule
dfs & GIN(E) &    0.0 \text{\tiny $\pm$ 0.1} &    0.0 \text{\tiny $\pm$ 0.0} &    0.0 \text{\tiny $\pm$ 0.0} &    0.0 \text{\tiny $\pm$ 0.0} &    0.0 \text{\tiny $\pm$ 0.0} &    0.0 \text{\tiny $\pm$ 0.0} &    0.0 \text{\tiny $\pm$ 0.0} &    0.0 \text{\tiny $\pm$ 0.0} &   0.0 \text{\tiny $\pm$ 0.0} &   0.0 \text{\tiny $\pm$ 0.0} &    0.0 \text{\tiny $\pm$ 0.0} &    0.0 \text{\tiny $\pm$ 0.0} &    0.0 \text{\tiny $\pm$ 0.0} &  0.0 \text{\tiny $\pm$ 0.0} &  0.0 \text{\tiny $\pm$ 0.0} \\
        & RecGNN &    0.0 \text{\tiny $\pm$ 0.0} &    0.0 \text{\tiny $\pm$ 0.0} &    0.0 \text{\tiny $\pm$ 0.0} &    0.0 \text{\tiny $\pm$ 0.0} &    0.0 \text{\tiny $\pm$ 0.0} &    0.0 \text{\tiny $\pm$ 0.0} &    0.0 \text{\tiny $\pm$ 0.0} &    0.0 \text{\tiny $\pm$ 0.0} &   0.0 \text{\tiny $\pm$ 0.0} &   0.0 \text{\tiny $\pm$ 0.0} &    0.0 \text{\tiny $\pm$ 0.0} &    0.0 \text{\tiny $\pm$ 0.0} &    0.0 \text{\tiny $\pm$ 0.0} &  0.0 \text{\tiny $\pm$ 0.0} &  0.0 \text{\tiny $\pm$ 0.0} \\
dfs (H) & GIN(E) &    0.0 \text{\tiny $\pm$ 0.0} &    0.0 \text{\tiny $\pm$ 0.0} &    0.0 \text{\tiny $\pm$ 0.0} &    0.0 \text{\tiny $\pm$ 0.0} &    0.0 \text{\tiny $\pm$ 0.0} &    0.0 \text{\tiny $\pm$ 0.0} &    0.0 \text{\tiny $\pm$ 0.0} &    0.0 \text{\tiny $\pm$ 0.0} &   0.0 \text{\tiny $\pm$ 0.0} &   0.0 \text{\tiny $\pm$ 0.0} &    0.0 \text{\tiny $\pm$ 0.0} &    0.0 \text{\tiny $\pm$ 0.0} &    0.0 \text{\tiny $\pm$ 0.0} &  0.0 \text{\tiny $\pm$ 0.0} &  0.0 \text{\tiny $\pm$ 0.0} \\
        & RecGNN &    1.1 \text{\tiny $\pm$ 1.6} &    0.0 \text{\tiny $\pm$ 0.0} &    0.0 \text{\tiny $\pm$ 0.0} &    0.0 \text{\tiny $\pm$ 0.0} &    0.0 \text{\tiny $\pm$ 0.0} &    0.0 \text{\tiny $\pm$ 0.0} &    0.0 \text{\tiny $\pm$ 0.0} &    0.0 \text{\tiny $\pm$ 0.0} &   0.0 \text{\tiny $\pm$ 0.0} &   0.0 \text{\tiny $\pm$ 0.0} &    0.5 \text{\tiny $\pm$ 0.7} &    0.0 \text{\tiny $\pm$ 0.0} &    0.0 \text{\tiny $\pm$ 0.0} &  0.0 \text{\tiny $\pm$ 0.0} &  0.0 \text{\tiny $\pm$ 0.0} \\
\midrule
dijkstra & GIN(E) &   72.8 \text{\tiny $\pm$ 8.2} &    0.4 \text{\tiny $\pm$ 0.2} &    0.0 \text{\tiny $\pm$ 0.0} &    0.0 \text{\tiny $\pm$ 0.0} &    0.0 \text{\tiny $\pm$ 0.0} &  45.6 \text{\tiny $\pm$ 12.7} &    0.1 \text{\tiny $\pm$ 0.1} &    0.0 \text{\tiny $\pm$ 0.0} &   0.0 \text{\tiny $\pm$ 0.0} &   0.0 \text{\tiny $\pm$ 0.0} &   65.6 \text{\tiny $\pm$ 9.1} &    0.0 \text{\tiny $\pm$ 0.0} &    0.0 \text{\tiny $\pm$ 0.0} &  0.0 \text{\tiny $\pm$ 0.0} &  0.0 \text{\tiny $\pm$ 0.0} \\
        & RecGNN &   85.2 \text{\tiny $\pm$ 8.6} &   10.0 \text{\tiny $\pm$ 8.3} &    0.7 \text{\tiny $\pm$ 0.8} &    0.0 \text{\tiny $\pm$ 0.0} &    0.0 \text{\tiny $\pm$ 0.0} &  64.0 \text{\tiny $\pm$ 14.1} &   10.7 \text{\tiny $\pm$ 8.7} &    0.5 \text{\tiny $\pm$ 0.6} &   0.0 \text{\tiny $\pm$ 0.0} &   0.0 \text{\tiny $\pm$ 0.0} &   80.3 \text{\tiny $\pm$ 8.1} &    8.1 \text{\tiny $\pm$ 7.5} &    0.1 \text{\tiny $\pm$ 0.2} &  0.0 \text{\tiny $\pm$ 0.0} &  0.0 \text{\tiny $\pm$ 0.0} \\
dijkstra (H) & GIN(E) &   41.7 \text{\tiny $\pm$ 4.1} &    0.0 \text{\tiny $\pm$ 0.0} &    0.0 \text{\tiny $\pm$ 0.0} &    0.0 \text{\tiny $\pm$ 0.0} &    0.0 \text{\tiny $\pm$ 0.0} &   18.4 \text{\tiny $\pm$ 3.1} &    0.0 \text{\tiny $\pm$ 0.0} &    0.0 \text{\tiny $\pm$ 0.0} &   0.0 \text{\tiny $\pm$ 0.0} &   0.0 \text{\tiny $\pm$ 0.0} &   32.8 \text{\tiny $\pm$ 4.1} &    0.0 \text{\tiny $\pm$ 0.0} &    0.0 \text{\tiny $\pm$ 0.0} &  0.0 \text{\tiny $\pm$ 0.0} &  0.0 \text{\tiny $\pm$ 0.0} \\
        & RecGNN &   70.7 \text{\tiny $\pm$ 6.1} &    0.0 \text{\tiny $\pm$ 0.0} &    0.0 \text{\tiny $\pm$ 0.0} &    0.0 \text{\tiny $\pm$ 0.0} &    0.0 \text{\tiny $\pm$ 0.0} &   46.7 \text{\tiny $\pm$ 4.5} &    0.0 \text{\tiny $\pm$ 0.0} &    0.0 \text{\tiny $\pm$ 0.0} &   0.0 \text{\tiny $\pm$ 0.0} &   0.0 \text{\tiny $\pm$ 0.0} &   61.8 \text{\tiny $\pm$ 6.4} &    0.0 \text{\tiny $\pm$ 0.0} &    0.0 \text{\tiny $\pm$ 0.0} &  0.0 \text{\tiny $\pm$ 0.0} &  0.0 \text{\tiny $\pm$ 0.0} \\
\midrule
eccentricity & GIN(E) &  80.9 \text{\tiny $\pm$ 22.4} &  70.8 \text{\tiny $\pm$ 38.7} &  67.9 \text{\tiny $\pm$ 30.7} &  58.4 \text{\tiny $\pm$ 37.3} &  44.0 \text{\tiny $\pm$ 23.4} &  80.0 \text{\tiny $\pm$ 38.4} &   18.7 \text{\tiny $\pm$ 7.8} &  13.3 \text{\tiny $\pm$ 23.5} &   8.2 \text{\tiny $\pm$ 4.6} &   7.1 \text{\tiny $\pm$ 6.0} &  74.6 \text{\tiny $\pm$ 41.2} &  26.7 \text{\tiny $\pm$ 16.3} &  31.6 \text{\tiny $\pm$ 28.8} &  0.0 \text{\tiny $\pm$ 0.0} &  0.0 \text{\tiny $\pm$ 0.0} \\
        & RecGNN &   99.3 \text{\tiny $\pm$ 0.3} &   98.9 \text{\tiny $\pm$ 1.0} &   96.6 \text{\tiny $\pm$ 2.0} &   94.4 \text{\tiny $\pm$ 5.2} &  73.0 \text{\tiny $\pm$ 11.5} &   99.8 \text{\tiny $\pm$ 0.4} &  39.5 \text{\tiny $\pm$ 16.5} &  42.6 \text{\tiny $\pm$ 33.8} &  16.3 \text{\tiny $\pm$ 2.2} &   9.7 \text{\tiny $\pm$ 7.1} &   99.9 \text{\tiny $\pm$ 0.3} &  47.6 \text{\tiny $\pm$ 31.0} &  36.2 \text{\tiny $\pm$ 19.5} &  0.0 \text{\tiny $\pm$ 0.0} &  0.0 \text{\tiny $\pm$ 0.0} \\
eccentricity (H) & GIN(E) &   29.7 \text{\tiny $\pm$ 9.6} &  25.8 \text{\tiny $\pm$ 34.3} &  25.9 \text{\tiny $\pm$ 31.7} &  13.8 \text{\tiny $\pm$ 18.4} &  10.3 \text{\tiny $\pm$ 18.6} &   18.7 \text{\tiny $\pm$ 9.3} &  26.5 \text{\tiny $\pm$ 23.0} &  30.6 \text{\tiny $\pm$ 29.7} &   2.5 \text{\tiny $\pm$ 4.2} &   5.0 \text{\tiny $\pm$ 7.8} &  18.2 \text{\tiny $\pm$ 14.0} &  30.0 \text{\tiny $\pm$ 29.0} &    5.1 \text{\tiny $\pm$ 9.8} &  0.0 \text{\tiny $\pm$ 0.0} &  0.0 \text{\tiny $\pm$ 0.0} \\
        & RecGNN &   83.9 \text{\tiny $\pm$ 9.9} &  74.4 \text{\tiny $\pm$ 24.1} &  63.9 \text{\tiny $\pm$ 26.8} &  64.2 \text{\tiny $\pm$ 24.7} &  61.3 \text{\tiny $\pm$ 28.4} &  81.7 \text{\tiny $\pm$ 18.4} &  42.1 \text{\tiny $\pm$ 26.7} &  50.8 \text{\tiny $\pm$ 24.4} &   5.2 \text{\tiny $\pm$ 8.5} &  11.2 \text{\tiny $\pm$ 6.4} &  84.3 \text{\tiny $\pm$ 18.8} &  35.6 \text{\tiny $\pm$ 28.5} &    0.9 \text{\tiny $\pm$ 0.8} &  0.0 \text{\tiny $\pm$ 0.0} &  0.0 \text{\tiny $\pm$ 0.0} \\
\midrule
mis & GIN(E) &   17.0 \text{\tiny $\pm$ 7.4} &    0.2 \text{\tiny $\pm$ 0.3} &    0.0 \text{\tiny $\pm$ 0.0} &    0.0 \text{\tiny $\pm$ 0.0} &    0.0 \text{\tiny $\pm$ 0.0} &   20.1 \text{\tiny $\pm$ 6.3} &    0.1 \text{\tiny $\pm$ 0.2} &    0.0 \text{\tiny $\pm$ 0.0} &   0.0 \text{\tiny $\pm$ 0.0} &   0.0 \text{\tiny $\pm$ 0.0} &   17.4 \text{\tiny $\pm$ 5.9} &    0.2 \text{\tiny $\pm$ 0.3} &    0.0 \text{\tiny $\pm$ 0.0} &  0.0 \text{\tiny $\pm$ 0.0} &  0.0 \text{\tiny $\pm$ 0.0} \\
        & RecGNN &  55.3 \text{\tiny $\pm$ 11.5} &    6.6 \text{\tiny $\pm$ 6.0} &    0.9 \text{\tiny $\pm$ 1.3} &    0.0 \text{\tiny $\pm$ 0.0} &    0.0 \text{\tiny $\pm$ 0.0} &  55.0 \text{\tiny $\pm$ 11.2} &   10.1 \text{\tiny $\pm$ 7.9} &    1.6 \text{\tiny $\pm$ 2.2} &   0.0 \text{\tiny $\pm$ 0.0} &   0.0 \text{\tiny $\pm$ 0.0} &  55.1 \text{\tiny $\pm$ 11.5} &   11.4 \text{\tiny $\pm$ 6.9} &    1.4 \text{\tiny $\pm$ 1.1} &  0.0 \text{\tiny $\pm$ 0.0} &  0.0 \text{\tiny $\pm$ 0.0} \\
mis (H) & GIN(E) &    2.2 \text{\tiny $\pm$ 1.8} &    0.0 \text{\tiny $\pm$ 0.0} &    0.0 \text{\tiny $\pm$ 0.0} &    0.0 \text{\tiny $\pm$ 0.0} &    0.0 \text{\tiny $\pm$ 0.0} &    3.1 \text{\tiny $\pm$ 2.5} &    0.0 \text{\tiny $\pm$ 0.0} &    0.0 \text{\tiny $\pm$ 0.0} &   0.0 \text{\tiny $\pm$ 0.0} &   0.0 \text{\tiny $\pm$ 0.0} &    2.2 \text{\tiny $\pm$ 1.6} &    0.0 \text{\tiny $\pm$ 0.0} &    0.0 \text{\tiny $\pm$ 0.0} &  0.0 \text{\tiny $\pm$ 0.0} &  0.0 \text{\tiny $\pm$ 0.0} \\
        & RecGNN &   56.9 \text{\tiny $\pm$ 6.8} &    3.9 \text{\tiny $\pm$ 3.1} &    0.2 \text{\tiny $\pm$ 0.3} &    0.0 \text{\tiny $\pm$ 0.0} &    0.0 \text{\tiny $\pm$ 0.0} &   57.4 \text{\tiny $\pm$ 7.8} &    9.0 \text{\tiny $\pm$ 5.6} &    1.2 \text{\tiny $\pm$ 1.0} &   0.0 \text{\tiny $\pm$ 0.0} &   0.0 \text{\tiny $\pm$ 0.0} &   58.5 \text{\tiny $\pm$ 8.8} &    8.6 \text{\tiny $\pm$ 3.4} &    0.7 \text{\tiny $\pm$ 0.5} &  0.0 \text{\tiny $\pm$ 0.0} &  0.0 \text{\tiny $\pm$ 0.0} \\
\midrule
mst & GIN(E) &   45.0 \text{\tiny $\pm$ 9.0} &    0.0 \text{\tiny $\pm$ 0.0} &    0.0 \text{\tiny $\pm$ 0.0} &    0.0 \text{\tiny $\pm$ 0.0} &    0.0 \text{\tiny $\pm$ 0.0} &   36.1 \text{\tiny $\pm$ 8.4} &    0.0 \text{\tiny $\pm$ 0.0} &    0.0 \text{\tiny $\pm$ 0.0} &   0.0 \text{\tiny $\pm$ 0.0} &   0.0 \text{\tiny $\pm$ 0.0} &   45.0 \text{\tiny $\pm$ 9.4} &    0.0 \text{\tiny $\pm$ 0.0} &    0.0 \text{\tiny $\pm$ 0.0} &  0.0 \text{\tiny $\pm$ 0.0} &  0.0 \text{\tiny $\pm$ 0.0} \\
        & RecGNN &  42.1 \text{\tiny $\pm$ 27.6} &    0.6 \text{\tiny $\pm$ 1.2} &    0.0 \text{\tiny $\pm$ 0.0} &    0.0 \text{\tiny $\pm$ 0.0} &    0.0 \text{\tiny $\pm$ 0.0} &  30.1 \text{\tiny $\pm$ 22.3} &    0.0 \text{\tiny $\pm$ 0.1} &    0.0 \text{\tiny $\pm$ 0.0} &   0.0 \text{\tiny $\pm$ 0.0} &   0.0 \text{\tiny $\pm$ 0.0} &  42.5 \text{\tiny $\pm$ 27.1} &    0.0 \text{\tiny $\pm$ 0.0} &    0.0 \text{\tiny $\pm$ 0.0} &  0.0 \text{\tiny $\pm$ 0.0} &  0.0 \text{\tiny $\pm$ 0.0} \\
mst (H) & GIN(E) &   28.5 \text{\tiny $\pm$ 5.7} &    0.0 \text{\tiny $\pm$ 0.0} &    0.0 \text{\tiny $\pm$ 0.0} &    0.0 \text{\tiny $\pm$ 0.0} &    0.0 \text{\tiny $\pm$ 0.0} &   17.1 \text{\tiny $\pm$ 3.5} &    0.0 \text{\tiny $\pm$ 0.0} &    0.0 \text{\tiny $\pm$ 0.0} &   0.0 \text{\tiny $\pm$ 0.0} &   0.0 \text{\tiny $\pm$ 0.0} &   30.6 \text{\tiny $\pm$ 5.7} &    0.0 \text{\tiny $\pm$ 0.0} &    0.0 \text{\tiny $\pm$ 0.0} &  0.0 \text{\tiny $\pm$ 0.0} &  0.0 \text{\tiny $\pm$ 0.0} \\
        & RecGNN &   31.6 \text{\tiny $\pm$ 4.6} &    0.0 \text{\tiny $\pm$ 0.0} &    0.0 \text{\tiny $\pm$ 0.0} &    0.0 \text{\tiny $\pm$ 0.0} &    0.0 \text{\tiny $\pm$ 0.0} &   19.0 \text{\tiny $\pm$ 3.5} &    0.0 \text{\tiny $\pm$ 0.0} &    0.0 \text{\tiny $\pm$ 0.0} &   0.0 \text{\tiny $\pm$ 0.0} &   0.0 \text{\tiny $\pm$ 0.0} &   33.3 \text{\tiny $\pm$ 5.5} &    0.0 \text{\tiny $\pm$ 0.0} &    0.0 \text{\tiny $\pm$ 0.0} &  0.0 \text{\tiny $\pm$ 0.0} &  0.0 \text{\tiny $\pm$ 0.0} \\
\bottomrule
\end{tabular}
}

==> results/main_results_old.tex <==
\begin{tabular}{l@{\hspace{1em}}l@{\hspace{1em}}S[table-format=3.1]S[table-format=3.1]S[table-format=3.1]S[table-format=3.1]S[table-format=3.1]@{\hspace{1em}}S[table-format=3.1]S[table-format=3.1]S[table-format=3.1]S[table-format=3.1]S[table-format=3.1]@{\hspace{1em}}S[table-format=3.1]S[table-format=3.1]S[table-format=3.1]S[table-format=3.1]S[table-format=3.1]}
\toprule
{\tiny Graph Type}    &        & \multicolumn{5}{l}{ER} & \multicolumn{5}{l}{WS} & \multicolumn{5}{l}{Delaunay} \\
{\tiny n}    &        &   \multicolumn{1}{l}{16}   &  \multicolumn{1}{l}{80}   &  \multicolumn{1}{l}{160}  &  \multicolumn{1}{l}{800}  &  \multicolumn{1}{l}{1600}  &   \multicolumn{1}{l}{16}   &  \multicolumn{1}{l}{80}   &  \multicolumn{1}{l}{160}  &  \multicolumn{1}{l}{800}  &  \multicolumn{1}{l}{1600} &     \multicolumn{1}{l}{16}   &  \multicolumn{1}{l}{80}   &  \multicolumn{1}{l}{160}  &  \multicolumn{1}{l}{800}  &  \multicolumn{1}{l}{1600} \\
\midrule
\midrule
BFS & GIN(E) &  100.0 &  99.9 &  99.7 &  99.1 &  99.1 &  100.0 &  95.6 &  88.8 &  75.7 &  80.4 &    100.0 &  99.0 &  95.1 &  73.5 &  66.4 \\
{\tiny (Node Acc.)}    & RecGNN &  100.0 &  99.9 &  99.7 &  99.3 &  99.1 &  100.0 &  96.5 &  87.5 &  76.7 &  82.5 &    100.0 &  97.7 &  90.9 &  72.8 &  62.2 \\
\midrule
DFS & GIN(E) &   40.8 &  25.5 &  14.1 &  13.0 &  11.8 &   24.6 &  14.8 &  16.3 &  22.0 &  20.0 &     39.3 &  24.8 &  23.1 &  21.3 &  21.0 \\
{\tiny (Node Acc.)}       & RecGNN &   34.0 &  21.0 &  12.1 &  11.3 &  10.6 &   22.9 &  13.3 &  15.3 &  20.5 &  18.8 &     34.7 &  20.4 &  19.2 &  18.2 &  18.1 \\
\midrule
Dijkstra & GIN(E) &   97.9 &  89.8 &  83.4 &  75.2 &  71.8 &   94.2 &  86.7 &  80.9 &  61.2 &  51.3 &     97.3 &  83.1 &  72.4 &  48.8 &  41.6 \\
{\tiny (Node Acc.)}       & RecGNN &   98.9 &  92.7 &  86.3 &  77.3 &  74.3 &   96.7 &  93.8 &  91.2 &  76.1 &  70.3 &     98.6 &  93.6 &  87.9 &  58.5 &  48.1 \\
\midrule
Eccentricity & GIN(E) &   80.9 &  70.8 &  67.9 &  58.4 &  44.0 &   80.0 &  18.7 &  13.3 &   8.2 &   7.1 &     74.6 &  26.7 &  31.6 &   0.0 &   0.0 \\
{\tiny (Graph Acc.)}       & RecGNN &   99.3 &  98.9 &  96.6 &  94.4 &  73.0 &   99.8 &  39.5 &  42.6 &  16.3 &   9.7 &     99.9 &  47.6 &  36.2 &   0.0 &   0.0 \\
\midrule
MIS & GIN(E) &   71.2 &  59.9 &  62.7 &  44.5 &  53.1 &   69.5 &  74.6 &  73.9 &  64.9 &  65.1 &     74.1 &  73.4 &  72.3 &  68.3 &  66.9 \\
{\tiny (Node F1)}       & RecGNN &   87.0 &  76.6 &  78.5 &  59.5 &  69.3 &   84.2 &  86.6 &  85.4 &  79.5 &  79.4 &     88.8 &  87.2 &  85.9 &  84.6 &  83.4 \\
\midrule
MST & GIN(E) &   92.8 &  79.9 &  77.9 &  73.9 &  71.9 &   90.6 &  76.2 &  75.2 &  73.5 &  73.4 &     93.1 &  78.5 &  76.4 &  75.3 &  75.1 \\
{\tiny (Node Acc.)}      & RecGNN &   89.8 &  75.3 &  70.0 &  59.8 &  56.0 &   86.4 &  69.8 &  64.4 &  53.4 &  52.5 &     90.6 &  72.5 &  63.0 &  50.7 &  49.7 \\
\bottomrule
\end{tabular}


==> results/node_acc_old.tex <==
\resizebox{.9\textwidth}{!}{
\begin{tabular}{l@{\hspace{1em}}l@{\hspace{1em}}S[table-format=3.1]@{\hspace{2.5em}}S[table-format=3.1]@{\hspace{2.5em}}S[table-format=3.1]@{\hspace{2.5em}}S[table-format=3.1]@{\hspace{2.5em}}S[table-format=3.1]@{\hspace{4em}}S[table-format=3.1]@{\hspace{2.5em}}S[table-format=3.1]@{\hspace{2.5em}}S[table-format=3.1]@{\hspace{2.5em}}S[table-format=3.1]@{\hspace{2.5em}}S[table-format=3.1]@{\hspace{4em}}S[table-format=3.1]@{\hspace{2.5em}}S[table-format=3.1]@{\hspace{2.5em}}S[table-format=3.1]@{\hspace{2.5em}}S[table-format=3.1]@{\hspace{2.5em}}S[table-format=3.1]@{\hspace{2.5em}}}
\toprule
    &        & \multicolumn{5}{l}{ER} & \multicolumn{5}{l}{WS} & \multicolumn{5}{l}{Delaunay} \\
    &        &   \multicolumn{1}{l}{16}   &  \multicolumn{1}{l}{80}   &  \multicolumn{1}{l}{160}  &  \multicolumn{1}{l}{800}  &  \multicolumn{1}{l}{1600}  &   \multicolumn{1}{l}{16}   &  \multicolumn{1}{l}{80}   &  \multicolumn{1}{l}{160}  &  \multicolumn{1}{l}{800}  &  \multicolumn{1}{l}{1600} &     \multicolumn{1}{l}{16}   &  \multicolumn{1}{l}{80}   &  \multicolumn{1}{l}{160}  &  \multicolumn{1}{l}{800}  &  \multicolumn{1}{l}{1600} \\
\midrule
bfs & GIN(E) &  100.0 \text{\tiny $\pm$ 0.0} &   99.9 \text{\tiny $\pm$ 0.1} &   99.7 \text{\tiny $\pm$ 0.2} &   99.1 \text{\tiny $\pm$ 0.5} &   99.1 \text{\tiny $\pm$ 0.4} &  100.0 \text{\tiny $\pm$ 0.0} &   95.6 \text{\tiny $\pm$ 2.0} &   88.8 \text{\tiny $\pm$ 3.3} &   75.7 \text{\tiny $\pm$ 6.0} &   80.4 \text{\tiny $\pm$ 1.4} &  100.0 \text{\tiny $\pm$ 0.0} &   99.0 \text{\tiny $\pm$ 0.8} &   95.1 \text{\tiny $\pm$ 3.8} &  73.5 \text{\tiny $\pm$ 24.0} &  66.4 \text{\tiny $\pm$ 23.4} \\
        & RecGNN &  100.0 \text{\tiny $\pm$ 0.0} &   99.9 \text{\tiny $\pm$ 0.1} &   99.7 \text{\tiny $\pm$ 0.1} &   99.3 \text{\tiny $\pm$ 0.1} &   99.1 \text{\tiny $\pm$ 0.2} &  100.0 \text{\tiny $\pm$ 0.0} &   96.5 \text{\tiny $\pm$ 1.7} &   87.5 \text{\tiny $\pm$ 6.8} &  76.7 \text{\tiny $\pm$ 10.4} &   82.5 \text{\tiny $\pm$ 1.5} &  100.0 \text{\tiny $\pm$ 0.0} &   97.7 \text{\tiny $\pm$ 2.3} &   90.9 \text{\tiny $\pm$ 9.0} &  72.8 \text{\tiny $\pm$ 22.4} &  62.2 \text{\tiny $\pm$ 22.5} \\
bfs (H) & GIN(E) &   98.4 \text{\tiny $\pm$ 3.4} &  94.7 \text{\tiny $\pm$ 10.4} &  93.9 \text{\tiny $\pm$ 11.5} &  88.5 \text{\tiny $\pm$ 21.9} &  84.8 \text{\tiny $\pm$ 25.8} &   98.6 \text{\tiny $\pm$ 2.9} &  79.4 \text{\tiny $\pm$ 22.5} &  61.9 \text{\tiny $\pm$ 19.0} &  44.3 \text{\tiny $\pm$ 22.3} &  61.6 \text{\tiny $\pm$ 28.3} &   97.4 \text{\tiny $\pm$ 5.5} &  80.6 \text{\tiny $\pm$ 24.9} &  66.2 \text{\tiny $\pm$ 22.4} &  41.6 \text{\tiny $\pm$ 18.4} &  35.0 \text{\tiny $\pm$ 16.0} \\
        & RecGNN &  100.0 \text{\tiny $\pm$ 0.0} &   99.0 \text{\tiny $\pm$ 0.5} &   98.3 \text{\tiny $\pm$ 1.0} &   97.3 \text{\tiny $\pm$ 1.3} &   94.1 \text{\tiny $\pm$ 1.5} &   99.9 \text{\tiny $\pm$ 0.1} &   89.9 \text{\tiny $\pm$ 2.4} &   79.0 \text{\tiny $\pm$ 7.7} &   53.9 \text{\tiny $\pm$ 6.2} &   64.8 \text{\tiny $\pm$ 7.9} &   99.9 \text{\tiny $\pm$ 0.1} &   85.7 \text{\tiny $\pm$ 3.1} &   67.0 \text{\tiny $\pm$ 4.0} &   39.2 \text{\tiny $\pm$ 2.3} &   33.6 \text{\tiny $\pm$ 1.2} \\
\midrule
dfs & GIN(E) &   40.8 \text{\tiny $\pm$ 9.0} &   25.5 \text{\tiny $\pm$ 6.4} &   14.1 \text{\tiny $\pm$ 5.5} &   13.0 \text{\tiny $\pm$ 5.7} &   11.8 \text{\tiny $\pm$ 5.0} &   24.6 \text{\tiny $\pm$ 4.4} &   14.8 \text{\tiny $\pm$ 0.9} &   16.3 \text{\tiny $\pm$ 0.5} &   22.0 \text{\tiny $\pm$ 0.6} &   20.0 \text{\tiny $\pm$ 0.5} &   39.3 \text{\tiny $\pm$ 9.8} &   24.8 \text{\tiny $\pm$ 6.1} &   23.1 \text{\tiny $\pm$ 6.0} &   21.3 \text{\tiny $\pm$ 6.0} &   21.0 \text{\tiny $\pm$ 6.0} \\
        & RecGNN &  34.0 \text{\tiny $\pm$ 13.2} &   21.0 \text{\tiny $\pm$ 8.7} &   12.1 \text{\tiny $\pm$ 7.4} &   11.3 \text{\tiny $\pm$ 7.2} &   10.6 \text{\tiny $\pm$ 6.4} &  22.9 \text{\tiny $\pm$ 11.3} &   13.3 \text{\tiny $\pm$ 2.0} &   15.3 \text{\tiny $\pm$ 1.5} &   20.5 \text{\tiny $\pm$ 1.8} &   18.8 \text{\tiny $\pm$ 1.5} &  34.7 \text{\tiny $\pm$ 12.9} &   20.4 \text{\tiny $\pm$ 9.0} &   19.2 \text{\tiny $\pm$ 8.3} &   18.2 \text{\tiny $\pm$ 7.9} &   18.1 \text{\tiny $\pm$ 7.9} \\
dfs (H) & GIN(E) &  42.4 \text{\tiny $\pm$ 10.1} &   27.3 \text{\tiny $\pm$ 6.5} &   18.0 \text{\tiny $\pm$ 5.4} &   17.2 \text{\tiny $\pm$ 5.1} &   15.6 \text{\tiny $\pm$ 4.5} &   26.8 \text{\tiny $\pm$ 4.4} &   15.7 \text{\tiny $\pm$ 1.4} &   16.8 \text{\tiny $\pm$ 0.6} &   22.0 \text{\tiny $\pm$ 1.0} &   20.0 \text{\tiny $\pm$ 0.8} &  41.1 \text{\tiny $\pm$ 10.6} &   25.8 \text{\tiny $\pm$ 6.9} &   25.3 \text{\tiny $\pm$ 5.0} &   24.6 \text{\tiny $\pm$ 4.2} &   24.4 \text{\tiny $\pm$ 4.2} \\
        & RecGNN &  46.0 \text{\tiny $\pm$ 16.7} &   26.0 \text{\tiny $\pm$ 6.6} &   17.1 \text{\tiny $\pm$ 5.2} &   15.9 \text{\tiny $\pm$ 5.0} &   14.5 \text{\tiny $\pm$ 4.6} &  33.9 \text{\tiny $\pm$ 14.6} &   16.0 \text{\tiny $\pm$ 1.9} &   16.8 \text{\tiny $\pm$ 1.0} &   21.8 \text{\tiny $\pm$ 1.1} &   19.8 \text{\tiny $\pm$ 0.9} &  46.1 \text{\tiny $\pm$ 18.7} &   25.8 \text{\tiny $\pm$ 5.9} &   24.4 \text{\tiny $\pm$ 5.2} &   23.4 \text{\tiny $\pm$ 5.1} &   23.3 \text{\tiny $\pm$ 5.1} \\
\midrule
dijkstra & GIN(E) &   97.9 \text{\tiny $\pm$ 0.8} &   89.8 \text{\tiny $\pm$ 2.6} &   83.4 \text{\tiny $\pm$ 4.9} &   75.2 \text{\tiny $\pm$ 5.8} &   71.8 \text{\tiny $\pm$ 7.0} &   94.2 \text{\tiny $\pm$ 2.8} &   86.7 \text{\tiny $\pm$ 0.7} &   80.9 \text{\tiny $\pm$ 1.9} &   61.2 \text{\tiny $\pm$ 3.9} &   51.3 \text{\tiny $\pm$ 5.9} &   97.3 \text{\tiny $\pm$ 0.9} &   83.1 \text{\tiny $\pm$ 0.8} &   72.4 \text{\tiny $\pm$ 2.8} &   48.8 \text{\tiny $\pm$ 3.3} &   41.6 \text{\tiny $\pm$ 1.5} \\
        & RecGNN &   98.9 \text{\tiny $\pm$ 0.7} &   92.7 \text{\tiny $\pm$ 5.6} &  86.3 \text{\tiny $\pm$ 10.1} &  77.3 \text{\tiny $\pm$ 13.9} &  74.3 \text{\tiny $\pm$ 13.9} &   96.7 \text{\tiny $\pm$ 2.0} &   93.8 \text{\tiny $\pm$ 5.1} &   91.2 \text{\tiny $\pm$ 6.8} &   76.1 \text{\tiny $\pm$ 9.8} &  70.3 \text{\tiny $\pm$ 10.5} &   98.6 \text{\tiny $\pm$ 0.6} &   93.6 \text{\tiny $\pm$ 6.1} &   87.9 \text{\tiny $\pm$ 8.6} &   58.5 \text{\tiny $\pm$ 5.5} &   48.1 \text{\tiny $\pm$ 2.7} \\
dijkstra (H) & GIN(E) &   94.3 \text{\tiny $\pm$ 0.7} &   71.5 \text{\tiny $\pm$ 1.0} &   60.8 \text{\tiny $\pm$ 1.5} &   51.9 \text{\tiny $\pm$ 3.2} &   49.1 \text{\tiny $\pm$ 2.6} &   89.2 \text{\tiny $\pm$ 1.8} &   65.8 \text{\tiny $\pm$ 3.3} &   57.7 \text{\tiny $\pm$ 4.5} &   40.3 \text{\tiny $\pm$ 5.9} &   34.1 \text{\tiny $\pm$ 6.8} &   93.1 \text{\tiny $\pm$ 0.8} &   61.7 \text{\tiny $\pm$ 4.1} &   47.9 \text{\tiny $\pm$ 5.6} &   33.4 \text{\tiny $\pm$ 7.7} &   31.0 \text{\tiny $\pm$ 8.3} \\
        & RecGNN &   97.6 \text{\tiny $\pm$ 0.7} &   38.4 \text{\tiny $\pm$ 5.8} &   27.6 \text{\tiny $\pm$ 7.5} &   17.1 \text{\tiny $\pm$ 5.8} &   15.8 \text{\tiny $\pm$ 5.4} &   94.8 \text{\tiny $\pm$ 0.9} &   35.3 \text{\tiny $\pm$ 3.8} &   29.4 \text{\tiny $\pm$ 6.1} &   26.4 \text{\tiny $\pm$ 5.9} &   25.3 \text{\tiny $\pm$ 6.0} &   96.9 \text{\tiny $\pm$ 0.8} &   38.3 \text{\tiny $\pm$ 5.4} &   31.2 \text{\tiny $\pm$ 7.2} &   27.3 \text{\tiny $\pm$ 7.3} &   26.8 \text{\tiny $\pm$ 7.2} \\
\midrule
mis & GIN(E) &   86.2 \text{\tiny $\pm$ 2.5} &   84.2 \text{\tiny $\pm$ 1.9} &   83.9 \text{\tiny $\pm$ 2.5} &   83.9 \text{\tiny $\pm$ 1.2} &   82.8 \text{\tiny $\pm$ 2.1} &   88.2 \text{\tiny $\pm$ 1.6} &   86.8 \text{\tiny $\pm$ 2.3} &   87.1 \text{\tiny $\pm$ 2.0} &   87.4 \text{\tiny $\pm$ 2.0} &   86.8 \text{\tiny $\pm$ 2.2} &   87.3 \text{\tiny $\pm$ 2.0} &   87.4 \text{\tiny $\pm$ 2.6} &   86.9 \text{\tiny $\pm$ 2.5} &   85.3 \text{\tiny $\pm$ 3.1} &   84.8 \text{\tiny $\pm$ 3.4} \\
        & RecGNN &   93.5 \text{\tiny $\pm$ 1.8} &   90.1 \text{\tiny $\pm$ 2.3} &   90.3 \text{\tiny $\pm$ 2.2} &   87.8 \text{\tiny $\pm$ 2.4} &   88.2 \text{\tiny $\pm$ 2.8} &   93.7 \text{\tiny $\pm$ 1.5} &   93.0 \text{\tiny $\pm$ 2.0} &   92.8 \text{\tiny $\pm$ 2.3} &   92.2 \text{\tiny $\pm$ 2.9} &   91.8 \text{\tiny $\pm$ 3.1} &   94.3 \text{\tiny $\pm$ 1.4} &   93.7 \text{\tiny $\pm$ 1.4} &   93.2 \text{\tiny $\pm$ 1.5} &   92.5 \text{\tiny $\pm$ 2.0} &   92.0 \text{\tiny $\pm$ 2.4} \\
mis (H) & GIN(E) &   77.2 \text{\tiny $\pm$ 2.5} &   77.9 \text{\tiny $\pm$ 4.5} &   76.6 \text{\tiny $\pm$ 4.6} &  76.3 \text{\tiny $\pm$ 16.3} &  73.9 \text{\tiny $\pm$ 13.0} &   80.8 \text{\tiny $\pm$ 2.3} &   77.0 \text{\tiny $\pm$ 2.0} &   78.3 \text{\tiny $\pm$ 2.3} &  77.5 \text{\tiny $\pm$ 10.6} &   77.5 \text{\tiny $\pm$ 9.0} &   77.7 \text{\tiny $\pm$ 2.5} &   78.6 \text{\tiny $\pm$ 1.7} &   78.5 \text{\tiny $\pm$ 2.3} &   75.2 \text{\tiny $\pm$ 7.4} &   75.1 \text{\tiny $\pm$ 7.0} \\
        & RecGNN &   93.0 \text{\tiny $\pm$ 1.6} &   89.0 \text{\tiny $\pm$ 1.7} &   88.9 \text{\tiny $\pm$ 2.0} &   86.3 \text{\tiny $\pm$ 1.9} &   86.2 \text{\tiny $\pm$ 2.5} &   93.3 \text{\tiny $\pm$ 1.7} &   92.7 \text{\tiny $\pm$ 2.3} &   92.3 \text{\tiny $\pm$ 2.6} &   91.1 \text{\tiny $\pm$ 3.1} &   90.4 \text{\tiny $\pm$ 3.3} &   94.2 \text{\tiny $\pm$ 1.7} &   92.9 \text{\tiny $\pm$ 1.8} &   92.3 \text{\tiny $\pm$ 2.1} &   91.0 \text{\tiny $\pm$ 2.7} &   90.2 \text{\tiny $\pm$ 3.1} \\
\midrule
mst & GIN(E) &   92.8 \text{\tiny $\pm$ 1.4} &   79.9 \text{\tiny $\pm$ 1.8} &   77.9 \text{\tiny $\pm$ 2.0} &   73.9 \text{\tiny $\pm$ 2.5} &   71.9 \text{\tiny $\pm$ 2.9} &   90.6 \text{\tiny $\pm$ 1.8} &   76.2 \text{\tiny $\pm$ 1.3} &   75.2 \text{\tiny $\pm$ 1.3} &   73.5 \text{\tiny $\pm$ 1.3} &   73.4 \text{\tiny $\pm$ 1.4} &   93.1 \text{\tiny $\pm$ 1.3} &   78.5 \text{\tiny $\pm$ 1.0} &   76.4 \text{\tiny $\pm$ 1.2} &   75.3 \text{\tiny $\pm$ 1.4} &   75.1 \text{\tiny $\pm$ 1.5} \\
        & RecGNN &   89.8 \text{\tiny $\pm$ 8.4} &  75.3 \text{\tiny $\pm$ 13.9} &  70.0 \text{\tiny $\pm$ 14.7} &  59.8 \text{\tiny $\pm$ 16.6} &  56.0 \text{\tiny $\pm$ 17.0} &  86.4 \text{\tiny $\pm$ 10.3} &  69.8 \text{\tiny $\pm$ 13.2} &  64.4 \text{\tiny $\pm$ 13.9} &  53.4 \text{\tiny $\pm$ 13.9} &  52.5 \text{\tiny $\pm$ 11.6} &   90.6 \text{\tiny $\pm$ 7.7} &  72.5 \text{\tiny $\pm$ 12.4} &  63.0 \text{\tiny $\pm$ 13.2} &  50.7 \text{\tiny $\pm$ 11.3} &  49.7 \text{\tiny $\pm$ 10.2} \\
mst (H) & GIN(E) &   89.9 \text{\tiny $\pm$ 1.0} &   61.5 \text{\tiny $\pm$ 7.0} &   59.2 \text{\tiny $\pm$ 7.3} &   54.4 \text{\tiny $\pm$ 8.3} &   51.7 \text{\tiny $\pm$ 8.4} &   85.9 \text{\tiny $\pm$ 1.7} &   62.6 \text{\tiny $\pm$ 4.5} &   60.7 \text{\tiny $\pm$ 4.2} &   58.8 \text{\tiny $\pm$ 4.4} &   60.7 \text{\tiny $\pm$ 3.8} &   90.5 \text{\tiny $\pm$ 1.0} &   65.4 \text{\tiny $\pm$ 4.1} &   63.7 \text{\tiny $\pm$ 3.8} &   62.6 \text{\tiny $\pm$ 3.5} &   62.5 \text{\tiny $\pm$ 3.4} \\
        & RecGNN &   89.8 \text{\tiny $\pm$ 1.1} &   29.0 \text{\tiny $\pm$ 8.0} &   25.5 \text{\tiny $\pm$ 6.2} &   19.3 \text{\tiny $\pm$ 7.3} &   18.1 \text{\tiny $\pm$ 6.9} &   84.9 \text{\tiny $\pm$ 1.3} &  31.9 \text{\tiny $\pm$ 10.5} &   27.6 \text{\tiny $\pm$ 5.0} &   22.7 \text{\tiny $\pm$ 6.7} &   25.1 \text{\tiny $\pm$ 8.4} &   90.5 \text{\tiny $\pm$ 1.2} &  34.3 \text{\tiny $\pm$ 12.9} &   31.7 \text{\tiny $\pm$ 9.0} &  27.4 \text{\tiny $\pm$ 10.6} &  27.3 \text{\tiny $\pm$ 10.6} \\
\bottomrule
\end{tabular}
}

==> results/node_f1.tex <==
\begin{tabular}{lllllllllllllllll}
\toprule
        &        & \multicolumn{5}{l}{ER} & \multicolumn{5}{l}{WS} & \multicolumn{5}{l}{Delaunay} \\
        &        &                          16   &                          80   &                          160  &                          800  &                          1600 &                          16   &                          80   &                          160  &                          800  &                          1600 &                          16   &                          80   &                          160  &                          800  &                          1600 \\
\midrule
MIS & GIN(E) &   61.2 \text{\tiny $\pm$ 7.0} &  48.2 \text{\tiny $\pm$ 11.1} &  51.7 \text{\tiny $\pm$ 11.1} &  29.5 \text{\tiny $\pm$ 17.2} &  41.1 \text{\tiny $\pm$ 14.6} &   57.5 \text{\tiny $\pm$ 7.2} &   63.5 \text{\tiny $\pm$ 7.1} &   61.7 \text{\tiny $\pm$ 8.6} &  52.7 \text{\tiny $\pm$ 12.8} &  53.2 \text{\tiny $\pm$ 13.1} &   62.7 \text{\tiny $\pm$ 8.3} &   60.5 \text{\tiny $\pm$ 7.8} &   58.1 \text{\tiny $\pm$ 9.7} &  56.5 \text{\tiny $\pm$ 11.1} &  55.2 \text{\tiny $\pm$ 11.6} \\
        & RecGNN &   87.7 \text{\tiny $\pm$ 4.3} &   76.5 \text{\tiny $\pm$ 6.8} &   78.5 \text{\tiny $\pm$ 6.6} &  61.8 \text{\tiny $\pm$ 10.9} &   70.6 \text{\tiny $\pm$ 9.4} &   84.0 \text{\tiny $\pm$ 5.0} &   85.6 \text{\tiny $\pm$ 5.3} &   83.9 \text{\tiny $\pm$ 6.7} &  77.5 \text{\tiny $\pm$ 10.5} &  77.9 \text{\tiny $\pm$ 10.4} &   89.3 \text{\tiny $\pm$ 3.6} &   86.5 \text{\tiny $\pm$ 4.5} &   85.5 \text{\tiny $\pm$ 5.9} &   84.3 \text{\tiny $\pm$ 7.3} &   83.4 \text{\tiny $\pm$ 8.2} \\
MIS (H) & GIN(E) &  52.1 \text{\tiny $\pm$ 14.2} &  26.8 \text{\tiny $\pm$ 17.7} &  29.4 \text{\tiny $\pm$ 18.1} &    9.5 \text{\tiny $\pm$ 8.1} &  18.3 \text{\tiny $\pm$ 13.7} &  50.8 \text{\tiny $\pm$ 13.1} &  50.5 \text{\tiny $\pm$ 17.4} &  45.1 \text{\tiny $\pm$ 20.1} &  34.0 \text{\tiny $\pm$ 19.9} &  32.5 \text{\tiny $\pm$ 19.9} &  56.5 \text{\tiny $\pm$ 14.0} &  46.3 \text{\tiny $\pm$ 20.0} &  40.9 \text{\tiny $\pm$ 22.4} &  37.0 \text{\tiny $\pm$ 23.1} &  35.0 \text{\tiny $\pm$ 22.9} \\
        & RecGNN &   84.9 \text{\tiny $\pm$ 1.0} &   73.5 \text{\tiny $\pm$ 5.2} &   74.4 \text{\tiny $\pm$ 8.0} &  51.8 \text{\tiny $\pm$ 19.0} &  60.1 \text{\tiny $\pm$ 19.3} &   82.4 \text{\tiny $\pm$ 1.1} &   85.2 \text{\tiny $\pm$ 3.5} &   83.7 \text{\tiny $\pm$ 5.2} &  75.2 \text{\tiny $\pm$ 11.5} &  72.1 \text{\tiny $\pm$ 15.8} &   87.5 \text{\tiny $\pm$ 1.0} &   84.9 \text{\tiny $\pm$ 2.9} &   83.4 \text{\tiny $\pm$ 4.7} &  79.0 \text{\tiny $\pm$ 10.3} &  75.1 \text{\tiny $\pm$ 15.0} \\
\bottomrule
\end{tabular}


==> results/node_f1_old.tex <==
\begin{tabular}{l@{\hspace{1em}}l@{\hspace{1em}}S[table-format=3.1]@{\hspace{2.5em}}S[table-format=3.1]@{\hspace{2.5em}}S[table-format=3.1]@{\hspace{2.5em}}S[table-format=3.1]@{\hspace{2.5em}}S[table-format=3.1]@{\hspace{4em}}S[table-format=3.1]@{\hspace{2.5em}}S[table-format=3.1]@{\hspace{2.5em}}S[table-format=3.1]@{\hspace{2.5em}}S[table-format=3.1]@{\hspace{2.5em}}S[table-format=3.1]@{\hspace{4em}}S[table-format=3.1]@{\hspace{2.5em}}S[table-format=3.1]@{\hspace{2.5em}}S[table-format=3.1]@{\hspace{2.5em}}S[table-format=3.1]@{\hspace{2.5em}}S[table-format=3.1]@{\hspace{2.5em}}}
\toprule
    &        & \multicolumn{5}{l}{ER} & \multicolumn{5}{l}{WS} & \multicolumn{5}{l}{Delaunay} \\
    &        &   \multicolumn{1}{l}{16}   &  \multicolumn{1}{l}{80}   &  \multicolumn{1}{l}{160}  &  \multicolumn{1}{l}{800}  &  \multicolumn{1}{l}{1600}  &   \multicolumn{1}{l}{16}   &  \multicolumn{1}{l}{80}   &  \multicolumn{1}{l}{160}  &  \multicolumn{1}{l}{800}  &  \multicolumn{1}{l}{1600} &     \multicolumn{1}{l}{16}   &  \multicolumn{1}{l}{80}   &  \multicolumn{1}{l}{160}  &  \multicolumn{1}{l}{800}  &  \multicolumn{1}{l}{1600} \\
\midrule
bfs & GIN(E) &  100.0 \text{\tiny $\pm$ 0.0} &   99.9 \text{\tiny $\pm$ 0.1} &   99.8 \text{\tiny $\pm$ 0.1} &   99.6 \text{\tiny $\pm$ 0.3} &   99.5 \text{\tiny $\pm$ 0.2} &  100.0 \text{\tiny $\pm$ 0.0} &   97.7 \text{\tiny $\pm$ 1.0} &   94.0 \text{\tiny $\pm$ 1.9} &   85.9 \text{\tiny $\pm$ 4.0} &   89.1 \text{\tiny $\pm$ 0.8} &  100.0 \text{\tiny $\pm$ 0.0} &   99.5 \text{\tiny $\pm$ 0.4} &   97.4 \text{\tiny $\pm$ 2.0} &  82.6 \text{\tiny $\pm$ 18.5} &  77.6 \text{\tiny $\pm$ 19.4} \\
        & RecGNN &  100.0 \text{\tiny $\pm$ 0.0} &   99.9 \text{\tiny $\pm$ 0.0} &   99.8 \text{\tiny $\pm$ 0.1} &   99.7 \text{\tiny $\pm$ 0.1} &   99.6 \text{\tiny $\pm$ 0.1} &  100.0 \text{\tiny $\pm$ 0.0} &   98.2 \text{\tiny $\pm$ 0.9} &   92.8 \text{\tiny $\pm$ 4.2} &   85.8 \text{\tiny $\pm$ 7.2} &   90.4 \text{\tiny $\pm$ 0.9} &  100.0 \text{\tiny $\pm$ 0.0} &   98.8 \text{\tiny $\pm$ 1.2} &   95.0 \text{\tiny $\pm$ 5.1} &  82.6 \text{\tiny $\pm$ 15.2} &  74.7 \text{\tiny $\pm$ 16.9} \\
bfs (H) & GIN(E) &   99.1 \text{\tiny $\pm$ 2.0} &   96.8 \text{\tiny $\pm$ 6.5} &   96.3 \text{\tiny $\pm$ 7.2} &  92.3 \text{\tiny $\pm$ 15.2} &  89.3 \text{\tiny $\pm$ 19.8} &   99.2 \text{\tiny $\pm$ 1.7} &  86.4 \text{\tiny $\pm$ 17.3} &  73.6 \text{\tiny $\pm$ 16.6} &  57.5 \text{\tiny $\pm$ 23.5} &  72.0 \text{\tiny $\pm$ 29.2} &   98.6 \text{\tiny $\pm$ 3.1} &  87.0 \text{\tiny $\pm$ 19.1} &  77.3 \text{\tiny $\pm$ 19.9} &  56.5 \text{\tiny $\pm$ 20.8} &  49.9 \text{\tiny $\pm$ 19.4} \\
        & RecGNN &  100.0 \text{\tiny $\pm$ 0.0} &   99.5 \text{\tiny $\pm$ 0.3} &   99.1 \text{\tiny $\pm$ 0.5} &   98.6 \text{\tiny $\pm$ 0.7} &   96.9 \text{\tiny $\pm$ 0.8} &  100.0 \text{\tiny $\pm$ 0.1} &   94.5 \text{\tiny $\pm$ 1.4} &   87.6 \text{\tiny $\pm$ 5.2} &   69.2 \text{\tiny $\pm$ 5.6} &   78.3 \text{\tiny $\pm$ 5.9} &  100.0 \text{\tiny $\pm$ 0.0} &   92.1 \text{\tiny $\pm$ 1.8} &   80.0 \text{\tiny $\pm$ 2.9} &   56.2 \text{\tiny $\pm$ 2.4} &   50.2 \text{\tiny $\pm$ 1.3} \\
\midrule
dfs & GIN(E) &   56.2 \text{\tiny $\pm$ 9.1} &   39.5 \text{\tiny $\pm$ 7.8} &   24.2 \text{\tiny $\pm$ 8.0} &   22.6 \text{\tiny $\pm$ 8.5} &   20.5 \text{\tiny $\pm$ 7.6} &   38.6 \text{\tiny $\pm$ 5.6} &   25.3 \text{\tiny $\pm$ 1.4} &   27.3 \text{\tiny $\pm$ 0.7} &   35.8 \text{\tiny $\pm$ 0.8} &   33.0 \text{\tiny $\pm$ 0.7} &  55.1 \text{\tiny $\pm$ 10.3} &   39.3 \text{\tiny $\pm$ 7.8} &   37.1 \text{\tiny $\pm$ 7.9} &   34.7 \text{\tiny $\pm$ 8.2} &   34.4 \text{\tiny $\pm$ 8.2} \\
        & RecGNN &  48.4 \text{\tiny $\pm$ 14.7} &  33.4 \text{\tiny $\pm$ 11.0} &  20.8 \text{\tiny $\pm$ 10.9} &  19.7 \text{\tiny $\pm$ 10.8} &   18.5 \text{\tiny $\pm$ 9.7} &  35.5 \text{\tiny $\pm$ 14.9} &   23.0 \text{\tiny $\pm$ 3.0} &   25.9 \text{\tiny $\pm$ 2.1} &   33.7 \text{\tiny $\pm$ 2.5} &   31.3 \text{\tiny $\pm$ 2.1} &  49.6 \text{\tiny $\pm$ 13.9} &  33.0 \text{\tiny $\pm$ 11.7} &  31.6 \text{\tiny $\pm$ 11.0} &  30.2 \text{\tiny $\pm$ 10.7} &  30.1 \text{\tiny $\pm$ 10.6} \\
dfs (H) & GIN(E) &  57.8 \text{\tiny $\pm$ 10.5} &   41.8 \text{\tiny $\pm$ 8.2} &   29.9 \text{\tiny $\pm$ 8.1} &   29.0 \text{\tiny $\pm$ 7.7} &   26.4 \text{\tiny $\pm$ 6.9} &   41.4 \text{\tiny $\pm$ 5.4} &   26.6 \text{\tiny $\pm$ 2.1} &   28.1 \text{\tiny $\pm$ 0.9} &   35.8 \text{\tiny $\pm$ 1.3} &   33.1 \text{\tiny $\pm$ 1.1} &  56.8 \text{\tiny $\pm$ 11.2} &   40.5 \text{\tiny $\pm$ 8.9} &   40.0 \text{\tiny $\pm$ 6.4} &   39.3 \text{\tiny $\pm$ 5.5} &   39.0 \text{\tiny $\pm$ 5.4} \\
        & RecGNN &  60.1 \text{\tiny $\pm$ 15.7} &   40.2 \text{\tiny $\pm$ 8.7} &   28.7 \text{\tiny $\pm$ 7.9} &   27.1 \text{\tiny $\pm$ 7.7} &   24.9 \text{\tiny $\pm$ 7.2} &  48.4 \text{\tiny $\pm$ 16.3} &   27.1 \text{\tiny $\pm$ 2.8} &   28.2 \text{\tiny $\pm$ 1.6} &   35.5 \text{\tiny $\pm$ 1.4} &   32.9 \text{\tiny $\pm$ 1.1} &  60.1 \text{\tiny $\pm$ 17.2} &   40.4 \text{\tiny $\pm$ 7.6} &   38.9 \text{\tiny $\pm$ 6.9} &   37.7 \text{\tiny $\pm$ 6.9} &   37.6 \text{\tiny $\pm$ 6.9} \\
\midrule
dijkstra & GIN(E) &   98.9 \text{\tiny $\pm$ 0.4} &   94.5 \text{\tiny $\pm$ 1.5} &   90.8 \text{\tiny $\pm$ 3.1} &   85.7 \text{\tiny $\pm$ 3.9} &   83.3 \text{\tiny $\pm$ 4.9} &   96.9 \text{\tiny $\pm$ 1.6} &   92.8 \text{\tiny $\pm$ 0.4} &   89.3 \text{\tiny $\pm$ 1.2} &   75.3 \text{\tiny $\pm$ 3.0} &   67.2 \text{\tiny $\pm$ 5.0} &   98.6 \text{\tiny $\pm$ 0.5} &   90.7 \text{\tiny $\pm$ 0.5} &   83.8 \text{\tiny $\pm$ 2.0} &   65.5 \text{\tiny $\pm$ 2.9} &   58.7 \text{\tiny $\pm$ 1.5} \\
        & RecGNN &   99.4 \text{\tiny $\pm$ 0.4} &   96.0 \text{\tiny $\pm$ 3.2} &   92.2 \text{\tiny $\pm$ 6.3} &   86.5 \text{\tiny $\pm$ 9.4} &   84.3 \text{\tiny $\pm$ 9.7} &   98.2 \text{\tiny $\pm$ 1.1} &   96.7 \text{\tiny $\pm$ 2.9} &   95.3 \text{\tiny $\pm$ 3.9} &   85.4 \text{\tiny $\pm$ 6.7} &   81.5 \text{\tiny $\pm$ 7.6} &   99.3 \text{\tiny $\pm$ 0.3} &   96.6 \text{\tiny $\pm$ 3.4} &   93.3 \text{\tiny $\pm$ 5.2} &   73.6 \text{\tiny $\pm$ 4.5} &   64.9 \text{\tiny $\pm$ 2.4} \\
dijkstra (H) & GIN(E) &   96.9 \text{\tiny $\pm$ 0.4} &   83.0 \text{\tiny $\pm$ 0.7} &   75.3 \text{\tiny $\pm$ 1.3} &   68.2 \text{\tiny $\pm$ 2.7} &   65.7 \text{\tiny $\pm$ 2.4} &   94.1 \text{\tiny $\pm$ 1.1} &   78.9 \text{\tiny $\pm$ 2.4} &   72.6 \text{\tiny $\pm$ 3.7} &   57.0 \text{\tiny $\pm$ 6.0} &   50.4 \text{\tiny $\pm$ 7.7} &   96.3 \text{\tiny $\pm$ 0.4} &   75.9 \text{\tiny $\pm$ 3.1} &   64.4 \text{\tiny $\pm$ 5.1} &   49.6 \text{\tiny $\pm$ 8.8} &   46.8 \text{\tiny $\pm$ 9.9} \\
        & RecGNN &   98.7 \text{\tiny $\pm$ 0.4} &   54.7 \text{\tiny $\pm$ 6.0} &   42.4 \text{\tiny $\pm$ 9.5} &   28.7 \text{\tiny $\pm$ 8.7} &   26.8 \text{\tiny $\pm$ 8.2} &   97.2 \text{\tiny $\pm$ 0.5} &   51.7 \text{\tiny $\pm$ 4.1} &   44.9 \text{\tiny $\pm$ 7.4} &   41.3 \text{\tiny $\pm$ 7.5} &   40.0 \text{\tiny $\pm$ 7.6} &   98.4 \text{\tiny $\pm$ 0.4} &   55.0 \text{\tiny $\pm$ 5.6} &   47.0 \text{\tiny $\pm$ 8.5} &   42.4 \text{\tiny $\pm$ 9.2} &   41.9 \text{\tiny $\pm$ 9.2} \\
\midrule
mis & GIN(E) &   71.2 \text{\tiny $\pm$ 7.8} &  59.9 \text{\tiny $\pm$ 14.0} &  62.7 \text{\tiny $\pm$ 14.9} &  44.5 \text{\tiny $\pm$ 22.9} &  53.1 \text{\tiny $\pm$ 23.3} &   69.5 \text{\tiny $\pm$ 6.9} &   74.6 \text{\tiny $\pm$ 7.4} &   73.9 \text{\tiny $\pm$ 7.3} &  64.9 \text{\tiny $\pm$ 14.1} &  65.1 \text{\tiny $\pm$ 15.8} &   74.1 \text{\tiny $\pm$ 6.0} &   73.4 \text{\tiny $\pm$ 8.9} &   72.3 \text{\tiny $\pm$ 8.9} &  68.3 \text{\tiny $\pm$ 14.0} &  66.9 \text{\tiny $\pm$ 16.4} \\
        & RecGNN &   87.0 \text{\tiny $\pm$ 3.7} &   76.6 \text{\tiny $\pm$ 6.0} &   78.5 \text{\tiny $\pm$ 5.4} &  59.5 \text{\tiny $\pm$ 10.1} &   69.3 \text{\tiny $\pm$ 8.3} &   84.2 \text{\tiny $\pm$ 4.0} &   86.6 \text{\tiny $\pm$ 3.9} &   85.4 \text{\tiny $\pm$ 4.6} &   79.5 \text{\tiny $\pm$ 7.2} &   79.4 \text{\tiny $\pm$ 7.9} &   88.8 \text{\tiny $\pm$ 2.9} &   87.2 \text{\tiny $\pm$ 3.0} &   85.9 \text{\tiny $\pm$ 3.3} &   84.6 \text{\tiny $\pm$ 4.2} &   83.4 \text{\tiny $\pm$ 5.2} \\
mis (H) & GIN(E) &  43.8 \text{\tiny $\pm$ 15.9} &  33.1 \text{\tiny $\pm$ 13.6} &  36.4 \text{\tiny $\pm$ 16.1} &  13.8 \text{\tiny $\pm$ 15.4} &  23.4 \text{\tiny $\pm$ 18.1} &  39.9 \text{\tiny $\pm$ 16.3} &  48.6 \text{\tiny $\pm$ 11.2} &   50.1 \text{\tiny $\pm$ 9.8} &   37.4 \text{\tiny $\pm$ 8.9} &  37.5 \text{\tiny $\pm$ 11.2} &  45.6 \text{\tiny $\pm$ 17.9} &  45.5 \text{\tiny $\pm$ 10.1} &  46.1 \text{\tiny $\pm$ 10.5} &  40.6 \text{\tiny $\pm$ 16.0} &  38.8 \text{\tiny $\pm$ 18.7} \\
        & RecGNN &   86.9 \text{\tiny $\pm$ 3.0} &   74.6 \text{\tiny $\pm$ 4.4} &   76.0 \text{\tiny $\pm$ 4.7} &  53.4 \text{\tiny $\pm$ 13.7} &  63.7 \text{\tiny $\pm$ 10.6} &   83.9 \text{\tiny $\pm$ 4.0} &   86.2 \text{\tiny $\pm$ 4.2} &   84.8 \text{\tiny $\pm$ 4.8} &   76.5 \text{\tiny $\pm$ 7.2} &   76.0 \text{\tiny $\pm$ 7.5} &   89.0 \text{\tiny $\pm$ 3.2} &   86.0 \text{\tiny $\pm$ 3.4} &   84.5 \text{\tiny $\pm$ 4.0} &   81.9 \text{\tiny $\pm$ 5.1} &   80.1 \text{\tiny $\pm$ 5.9} \\
\midrule
mst & GIN(E) &   96.0 \text{\tiny $\pm$ 0.8} &   88.7 \text{\tiny $\pm$ 1.1} &   87.5 \text{\tiny $\pm$ 1.3} &   84.9 \text{\tiny $\pm$ 1.7} &   83.5 \text{\tiny $\pm$ 2.0} &   94.7 \text{\tiny $\pm$ 1.1} &   86.3 \text{\tiny $\pm$ 0.8} &   85.8 \text{\tiny $\pm$ 0.9} &   84.7 \text{\tiny $\pm$ 0.9} &   84.7 \text{\tiny $\pm$ 0.9} &   96.2 \text{\tiny $\pm$ 0.7} &   87.9 \text{\tiny $\pm$ 0.6} &   86.6 \text{\tiny $\pm$ 0.8} &   85.9 \text{\tiny $\pm$ 0.9} &   85.8 \text{\tiny $\pm$ 1.0} \\
        & RecGNN &   94.1 \text{\tiny $\pm$ 5.1} &   85.1 \text{\tiny $\pm$ 9.7} &  81.4 \text{\tiny $\pm$ 10.9} &  73.6 \text{\tiny $\pm$ 13.8} &  70.3 \text{\tiny $\pm$ 14.7} &   92.0 \text{\tiny $\pm$ 6.5} &   81.3 \text{\tiny $\pm$ 9.7} &  77.5 \text{\tiny $\pm$ 10.8} &  68.6 \text{\tiny $\pm$ 12.2} &  68.1 \text{\tiny $\pm$ 10.2} &   94.7 \text{\tiny $\pm$ 4.6} &   83.4 \text{\tiny $\pm$ 8.7} &  76.5 \text{\tiny $\pm$ 10.2} &   66.5 \text{\tiny $\pm$ 9.9} &   65.9 \text{\tiny $\pm$ 8.8} \\
mst (H) & GIN(E) &   94.4 \text{\tiny $\pm$ 0.6} &   75.7 \text{\tiny $\pm$ 5.6} &   73.9 \text{\tiny $\pm$ 6.1} &   69.8 \text{\tiny $\pm$ 7.3} &   67.4 \text{\tiny $\pm$ 7.8} &   92.0 \text{\tiny $\pm$ 1.0} &   76.7 \text{\tiny $\pm$ 3.4} &   75.3 \text{\tiny $\pm$ 3.2} &   73.9 \text{\tiny $\pm$ 3.4} &   75.5 \text{\tiny $\pm$ 2.9} &   94.7 \text{\tiny $\pm$ 0.6} &   78.9 \text{\tiny $\pm$ 3.0} &   77.7 \text{\tiny $\pm$ 2.8} &   77.0 \text{\tiny $\pm$ 2.7} &   76.9 \text{\tiny $\pm$ 2.6} \\
        & RecGNN &   94.3 \text{\tiny $\pm$ 0.6} &   44.1 \text{\tiny $\pm$ 9.1} &   39.9 \text{\tiny $\pm$ 7.9} &  31.6 \text{\tiny $\pm$ 10.3} &   29.8 \text{\tiny $\pm$ 9.9} &   91.3 \text{\tiny $\pm$ 0.8} &  47.3 \text{\tiny $\pm$ 11.5} &   42.8 \text{\tiny $\pm$ 6.2} &   36.4 \text{\tiny $\pm$ 8.8} &  39.3 \text{\tiny $\pm$ 10.8} &   94.7 \text{\tiny $\pm$ 0.7} &  49.8 \text{\tiny $\pm$ 13.9} &  47.5 \text{\tiny $\pm$ 10.6} &  42.1 \text{\tiny $\pm$ 13.5} &  42.0 \text{\tiny $\pm$ 13.6} \\
\bottomrule
\end{tabular}

